Ajalon: Simplifying the Authoring of Wearable Cognitive Assistants

Wearable Cognitive Assistance (WCA) amplifies human cognition in real time through a wearable device and low-latency wireless access to edge computing infrastructure. It is inspired by, and broadens, the metaphor of GPS navigation tools that provide real-time step-by-step guidance, with prompt error detection and correction. WCA applications are likely to be transformative in education, health care, industrial troubleshooting, manufacturing, and many other areas. Today, WCA application development is difficult and slow, requiring skills in areas such as machine learning and computer vision that are not widespread among software developers. This paper describes Ajalon, an authoring toolchain for WCA applications that reduces the skill and effort needed at each step of the development pipeline. Our evaluation shows that Ajalon significantly reduces the effort needed to create new WCA applications.

==> motivation.tex <==
\section{Motivation}
In Fig. \ref{fig:buildingprocess}, a typical flow of building a new application is characterized by consisting of four main components. First, domain experts explore all steps and    
\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.8\textwidth]{Figures/CognitiveAppBuildingProcess.png}
	\caption{Cognitive assistant application building process}
	\label{fig:buildingprocess}
\end{figure*}
